MathGLM-Vision: Solving Mathematical Problems with Multi-Modal Large Language Model

Large language models (LLMs) have demonstrated significant capabilities in mathematical reasoning, particularly with text-based mathematical problems. However, current multi-modal large language models (MLLMs), especially those specialized in mathematics, tend to focus predominantly on solving geometric problems but ignore the diversity of visual information available in other areas of mathematics. Moreover, the geometric information for these specialized mathematical MLLMs is derived from several public datasets, which are typically limited in diversity and complexity. To address these limitations, we aim to construct a fine-tuning dataset named MathVL, and develop a series of specialized mathematical MLLMs termed MathGLM-Vision by conducting Supervised Fine-Tuning (SFT) on MathVL with various parameter-scale backbones. To extensively evaluate the effectiveness of MathGLM-Vision, we conduct experiments on several public benchmarks and our curated MathVL-test consisting of 2,000 problems. Experimental results demonstrate that MathGLM-Vision achieves significant improvements compared with some existing models, including backbone models and open-source mathematical MLLMs. These findings indicate the importance of diversity dataset in enhancing the mathematical reasoning abilities of MLLMs.

==> copy.tex <==

% In this section, we evaluate various models including LLMs and MLLMs. For each type, we consider both closed- and open-source models. 

\subsection{Experimental Setup}



\vpara{Evaluation Datasets.} We assess our \model using three well-established public benchmark datasets(MathVista~\cite{lu2023mathvista}, MathVerse~\cite{zhang2024mathverse}, and Math-Vision~\cite{wang2024measuring} datasets) alongside our specially curated dataset \data-test. The \data-test dataset comprises 2,000 sampled cases, distinct from those in the \data dataset, ensuring a rigorous and unbiased evaluation of \model's capabilities. Furthermore, we adopt the testing protocol~\cite{gao2023g} and utilize MathVista-GPS dataset to evaluate \model's geometry problem solving ability. Additionally, we evaluate \model's enhanced general vision-language understanding skills using the MMMU benchmark~\cite{yue2024mmmu}. Detailed descriptions for these benchmark datasets are provided in Appendix~\ref{appendix: benchmark_dataset}.




% \vpara{Compared Models.} We compare \model with other models across three distinct categories: (a) Text-only Large Language Models (LLMs) only take textual questions as input, including ChatGPT~\cite{}, GPT-4~\cite{}, and Claude-2~\cite{} in zero-shot and two-shot settings with Chain-of-Thought (CoT)~\cite{} and Program-of-Thought (PoT)~\cite{}. (b) Closed-source Multi-Modal Large Language Models (MLLMs), represented by models like GPT-4V~\cite{}, Gemini-Pro~\cite{}, Gemini Ultra~\cite{}, Qwen-VL-Max~\cite{}, and Qwen-VL-Plus~\cite{}, and Multimodal Bard~\cite{}. (c) Open-source MLLMs, featuring models such as IDEFICS-9B~\cite{laurenccon2024obelics}, LLaVA~\cite{liu2024visual}(LLaMA2-13B~\cite{touvron2023llama2}), LLaVA-1.5~\cite{liu2024improved} (Vicuna-13B~\cite{chiang2023vicuna}), LLaVA-NeXT~\cite{liu2024llava} (Vicuna-13B), SPHINX-MoE~\cite{gao2024sphinx}(Mixtral-8×7B~\cite{jiang2024mixtral}), SPHINX-Plus (LLaMA2-13B), InternLM-XComposer2~\cite{dong2024internlm} (InternLM2-7B~\cite{team2023internlm}), LLaMA-Adapter V2~\cite{gao2023llama}(LLaMA-7B~\cite{touvron2023llama1}), ImageBind-LLM~\cite{han2023imagebind} (LLaMA-7B), MiniGPT-v2~\cite{chen2023minigpt} (LLaMA2-7B), mPLUG-Owl~\cite{ye2023mplug} (LLaMA-7B), mPLUG-Owl2~\cite{ye2024mplug} (LLaMA-7B), miniGPT4~\cite{zhu2023minigpt}, InstructBLIP~\cite{dai2024instructblip} (Vicuna-7B), LLaVAR~\cite{zhang2023llavar}, G-LLaVA-7B~\cite{gao2023g} (LLaMA2-7B), G-LLaVA-13B (LLaMA2-13B), InternVL-1.5~\cite{chen2024internvl}and ShareGPT-4V~\cite{chen2023sharegpt4v} (Vicuna-13B).


\vpara{Compared Models.} We compare \model with other Multi-Modal Large Language Models (MLLMs), including closed-source MLLMs and open-source MLLMs. Additionally, we compare \model with recent specialized mathematical MLLMs, including G-LLaVA~\cite{gao2023g}, GeoGPT4V~\cite{cai2024geogpt4v}, and Math-LLaVA~\cite{shihu2024mathllava}. 


% represented by models like GPT-4V~\cite{}, Gemini-Pro~\cite{}, Gemini Pro~\cite{}, Qwen-VL-Max~\cite{}, and Qwen-VL-Plus~\cite{}, and Multimodal Bard~\cite{}. (c) Open-source MLLMs, featuring models such as IDEFICS-9B~\cite{laurenccon2024obelics}, LLaVA~\cite{liu2024visual}(LLaMA2-13B~\cite{touvron2023llama2}), LLaVA-1.5~\cite{liu2024improved} (Vicuna-13B~\cite{chiang2023vicuna}), LLaVA-NeXT~\cite{liu2024llava} (Vicuna-13B), SPHINX-MoE~\cite{gao2024sphinx}(Mixtral-8×7B~\cite{jiang2024mixtral}), SPHINX-Plus (LLaMA2-13B), InternLM-XComposer2~\cite{dong2024internlm} (InternLM2-7B~\cite{team2023internlm}), LLaMA-Adapter V2~\cite{gao2023llama}(LLaMA-7B~\cite{touvron2023llama1}), ImageBind-LLM~\cite{han2023imagebind} (LLaMA-7B), MiniGPT-v2~\cite{chen2023minigpt} (LLaMA2-7B), mPLUG-Owl~\cite{ye2023mplug} (LLaMA-7B), mPLUG-Owl2~\cite{ye2024mplug} (LLaMA-7B), miniGPT4~\cite{zhu2023minigpt}, InstructBLIP~\cite{dai2024instructblip} (Vicuna-7B), LLaVAR~\cite{zhang2023llavar}, G-LLaVA-7B~\cite{gao2023g} (LLaMA2-7B), G-LLaVA-13B (LLaMA2-13B), InternVL-1.5~\cite{chen2024internvl}and ShareGPT-4V~\cite{chen2023sharegpt4v} (Vicuna-13B).


\vpara{Evaluation Metrics.} We adopt top-1 accuracy for evaluating our \model for MathVista, MathVerse, MathVision, and \data-test. For evaluation, we follow the evaluation pipeline proposed in abovementioned benchmark datasets, which first employs ChatGPT to extract the predicted answers from responses and then calculate accuracy by matching the ground truth and the extracted final answer.    


\subsection{Main Results}

\yz{done this -- 7.1}

We compare \model with other models on MathVista-GPS~\cite{lu2023mathvista}, minitest split of MathVista~\cite{lu2023mathvista}, MathVerse~\cite{zhang2024mathverse}, MathVision~\cite{wang2024measuring} benchmarks, and our curated Chinese benchmark \data on Table~\ref{tab:main_results}. \yz{write main results}

\begin{table*}[htbp]
    \centering
    \renewcommand{\arraystretch}{1.15}
    \small
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{cccccccc}  
    \toprule
     Model & Input & LLM Size  & MathVista-GPS & MathVista & MathVerse & MathVision  & \data \\
    \midrule
    \multicolumn{7}{c}{\textit{Closed Source Models (General Multimodal LLMs)}}\\
     \midrule
     Gemini Pro &    \textit{Q}, \textit{I} & - &   & 45.20 &  36.80  & 17.66 \\ 
     Gemini1.5 Pro &    \textit{Q}, \textit{I} & - &  & 63.90  &  &  19.24 & \\ 
     GPT-4V & \textit{Q}, \textit{I} & - & 50.5  & 49.90  &  50.80 & 22.76   & 35.89   \\ 
     GPT-4-turbo & \textit{Q}, \textit{I} & - &  \yz{done}  & 58.10 & \yz{done}  & 30.26 & 42.19  \\ 
     GPT-4o & \textit{Q}, \textit{I} & - & \yz{done}  & 63.80  & \yz{done}  & 30.39  &  51.05 \\ 
     Claude-3-opus & \textit{Q} & - &  & 50.50 &  &  &   \\
     Qwen-VL-Plus & \textit{Q}, \textit{I} & - &  & 43.30 & 19.10 & 10.72  & \JH{doing}    \\
     Qwen-VL-Max & \textit{Q}, \textit{I} & - &   & 51.00 & 35.90 &  15.59 & \JH{doing}   \\
     \midrule
    \multicolumn{7}{c}{\textit{Open Source Models }}\\
    \midrule
    \multicolumn{7}{l}{\textit{General Multimodal LLMs}}\\
    mPLUG-Owl  & \textit{Q}, \textit{I} & 7B & 23.60 & 22.20 & &   \\
    miniGPT4  & \textit{Q}, \textit{I} & 7B & 26.00 & 23.10 & &   \\
    LLaMA-Adapter-V2  & \textit{Q}, \textit{I} & 7B  & 25.50 & 23.90 & 4.50  &    \\
    InstructBLIP  & \textit{Q}, \textit{I} & 7B & 20.70 & 25.30 & &   \\
    LLaVA-1.5  & \textit{Q}, \textit{I} & 13B & 24.04  &  27.60 & 12.70 & 11.12   \\
    ShareGPT-4V & \textit{Q}, \textit{I} & 13B &  & 29.30 & 16.20 & 10.53   \\
    SPHINX-MoE & \textit{Q}, \textit{I} & 8*7B &  & 36.80 & 19.60 & 14.18\\
    SPHINX-Plus & \textit{Q}, \textit{I} & 13B &  & 36.70 & 14.70 & 9.70 \\
    InternLM-XC2  & \textit{Q}, \textit{I} & 7B & & 57.60 & 24.40 & 14.54 & \\
    InternVL-1.2-Plus & \textit{Q}, \textit{I} & 20B & & 59.90 &  & 16.97 &   \\
    \midrule
    \multicolumn{7}{l}{\textit{Geo-Multimodal LLMs}}\\
    G-LLaVA & \textit{Q}, \textit{I} & 7B & 53.40 & \yz{load model} & 12.70 &   \\
    G-LLaVA & \textit{Q}, \textit{I} & 13B & 56.70 & & \yz{load model}  & &    \\
    GeoGPT4V (LLaVA-1.5) & \textit{Q}, \textit{I} & 7B & 32.69 & \yz{no model release}  & &   \\
    GeoGPT4V (LLaVA-1.5) & \textit{Q}, \textit{I} & 13B  & 36.54 & \\
    GeoGPT4V (ShareGPT4V-G) & \textit{Q}, \textit{I} & 7B & 32.69  \\
    GeoGPT4V (ShareGPT4V-G) & \textit{Q}, \textit{I} & 13B & 43.27 \\
    Math-LLaVA  & \textit{Q}, \textit{I} & 13B &  & 46.60 & & 15.69 & \\
    \midrule
    \multicolumn{7}{c}{\textit{\model and Backbone Models}}\\
    \midrule
    GLM-4-V-9B-standard  & \textit{Q}, \textit{I} & 9B  & 40.38 &  44.30  & 34.77\JH{re}  & 25.13 & 30.59 \\
    \textbf{\model-9B} & \textit{Q}, \textit{I}  & 9B & 50.49  & 47.00 &  40.48\JH{re}  & 32.25  & 58.52 \\
    \hline
    CogVLM2-standard  & \textit{Q}, \textit{I} & 8B & 39.61  & 38.00 &  23.86\JH{re} &  21.70 & 27.47 \\
    \textbf{\model-19B} & \textit{Q}, \textit{I} & 8B & 55.07 & 63.20 & 45.94\JH{re} & 35.63 & 57.42 \\
    \hline
    CogVLM-32B-standard  & \textit{Q}, \textit{I}  & 32B & 36.59 & 44.50   & 30.20\JH{re}  & 17.17 & 30.86 \\
    \textbf{\model-32B} & \textit{Q}, \textit{I} & 32B & 56.25  & 71.30 & 44.67\JH{re} & 36.08 & 58.99  \\
    \bottomrule
    \end{tabular}} 
    \caption{\textbf{Results on several public benchmark datasets.} Comparison of model performance on the test-mini set of MathVista benchmarks~\cite{lu2023mathvista} on geometry problem solving (GPS). For input, $\textit{Q}$ represents for question, $\textit{I}$ represents for image. For MathVerse dataset, we only evaluate LLMs on Vision Dominant with CoT-E.}
    \label{tab:main_results}
\end{table*}


    % GLM-4-V-9B$^{*}$  & \textit{Q}, \textit{I} & 9B  & 43.75 &  42.40  & 16.62\JH{re}  & 12.11\JH{re} & 16.30 \\
    % CogVLM-32B  & \textit{Q}, \textit{I}  & 32B & 45.19 & 50.21   & 39.09  & 11.91\JH{re} & 34.45 \\
    % CogVLM2  & \textit{Q}, \textit{I} & 8B & 37.98  & 37.50 & 20.94  &  13.93 & 21.20 \\


 % \midrule
     %  \multicolumn{5}{l}{\textit{Visual-Augmented LLMs}}\\
     % 2-shot CoT Claude-2 & \textit{Q}, \textit{I}$_c$, \textit{I}$_t$ & 31.7  &  &  &     \\
     % 2-shot CoT ChatGPT &    \textit{Q}, \textit{I}$_c$, \textit{I}$_t$ & 29.3  &  &  &    \\ 
     % 2-shot CoT GPT-4 & \textit{Q}, \textit{I}$_c$, \textit{I}$_t$ & 31.7  &  &  &     \\ 
     % % \midrule
     % 2-shot PoT ChatGPT & \textit{Q}, \textit{I}$_c$, \textit{I}$_t$ & 26.4  &  &  &    \\ 
     % 2-shot PoT GPT-4 & \textit{Q}, \textit{I}$_c$, \textit{I}$_t$ & 39.4   &  &  &     \\ 

  % \midrule
     % 2-shot PoT ChatGPT & \textit{Q} & 30.8  & 25.1 &  &    \\ 
     % 2-shot PoT GPT-4 & \textit{Q} & 33.2   & 26.0 &   &    \\ 

    % \multicolumn{7}{c}{\textit{Heuristics Baseline}}\\
    % \midrule
    %  Random Chance & - & 21.6  & 17.9 &  -  & 7.17 &     \\
    %  Frequent Guess & - & 34.1  & 26.3  & -  & - &     \\ 
    %  Human & \textit{Q},  \textit{I} & 48.4  &  60.3  & -   & - &    \\ 
    %  \midrule
% \midrule
    % \multicolumn{7}{l}{\textit{Text-only LLMs}}\\
    %  Zero-shot ChatGPT & \textit{Q} & -  & 26.9  & 23.5  &  &    & 19.05 \yz{re} \\
    %  Zero-shot GPT-4 & \textit{Q} & - & 37.0  & 26.1 &  &   & 37.10 \yz{re}  \\ 
    %  % Zero-shot GPT-4o & \textit{Q} & - &    &  &  & \JH{doing}  & (\yz{re})   \\ 
    %  Zero-shot Claude-3-opus & \textit{Q} & - & 34.1   & 26.4 &   &    & \yz{by zhen} \\ 
    %  % \midrule
    %  2-shot CoT Claude-3-opus & \textit{Q} & - & 29.8  & 24.4 &  &  & \yz{by zhen}  \\
    %  2-shot CoT ChatGPT & \textit{Q} & - & 36.5  &  26.8 &     & 8.82 & 17.95  \\ 
    %  2-shot CoT GPT-4 & \textit{Q} & - & 44.7   & 29.2 &   & 19.08 & 36.55  \\ 
     % 2-shot CoT GPT-4o & \textit{Q} & - &    &  &  & \JH{doing}  & 41.55(\yz{re})   \\ 

\vpara{Results on the testmini subset of MathVista.} To comprehensively evaluate the performance of \model across various task types featured in the MathVista dataset, we systematically tested it on the Testmini subset. This subset has been carefully selected to represent a diverse range of mathematical problem types, ensuring a robust assessment of our model's capabilities. Table~\ref{tab:mathvista_test_result} shows the evaluation results on the testmini subset of MathVista across various task types. \yz{write the results.}


\begin{table*}[h]
\centering
 \small
 \renewcommand\arraystretch{1.15} % row space
\begin{adjustbox}{width=\linewidth}
    \begin{tabular}{l|c|c|ccccc|ccccccc}
    \toprule
    Model & Input & ALL & FQA & GPS& MWP & TQA & VQA & ALG & ARI & GEO & LOG & NUM & SCI& STA  \\ 
    \midrule
    Random chance & - & 17.86 & 15.46 & 24.12 & 4.54 & 23.36 & 24.33 & 25.84 & 13.85 & 22.69 & 13.40 & 8.82 & 15.76 & 14.28 \\
    Frequent guess & - & 23.48 & 20.97 & 27.18 & 16.27 & 26.06 & 28.87 & 28.29 & 20.86 & 25.71 & 11.86 & 19.61 & 20.45 & 20.08 \\
    \midrule
    2-shot CoT GPT-4 & $Q$, $I_c$, $I_t$ & 30.50 & 27.21 & 35.91 & 21.30 & 43.13 & 28.17 & 35.72 & 25.17 & 35.80 & 24.74 & 15.41 & 47.28 & 31.29 \\
    2-shot PoT GPT-4 & $Q$, $I_c$, $I_t$ & 31.74 & 27.58 & 37.35 & 23.87 & 43.00 & 30.27 & 37.15 & 27.93 & 37.48 & 22.68 & 15.83 & 44.47 & 31.87 \\
    \midrule
    LLaVA-LLaMA-2-13B & $Q$, $I$ & 25.40 & 22.86 & 24.57 & 18.15 & 35.82 & 29.69 & 26.93 & 22.47 & 24.45 & 19.07 & 19.05 & 34.71 & 21.61 \\
    \midrule 
    \textbf{\model-9B} & $Q$, $I$ & \\
    \textbf{\model-19B} & $Q$, $I$ & \\
    \textbf{\model-32B} & $Q$, $I$ &\\
    \bottomrule
    \end{tabular}
    \end{adjustbox}
    \caption{\textbf{Accuracy scores on the \textit{test} subset of MathVista.} Input: $Q$: question, $I$: image, $I_c$: image caption, $I_t$: OCR texts detected from the image. ALL: overall accuracy. Task types: FQA: figure question answering, GPS: geometry problem solving, MWP: math word problem, TQA: textbook question answering, VQA: visual question answering. Mathematical reasoning types: ALG: algebraic reasoning, ARI: arithmetic reasoning, GEO: geometry reasoning, LOG: logical reasoning, NUM: numeric common sense, SCI: scientific reasoning, STA: statistical reasoning.}
\label{tab:mathvista_test_result}
\end{table*}




\vpara{Results on the testmini set of MathVerse.} To thoroughly evaluate the performance of \model across 12 detailed subjects within the MathVerse dataset, we conduct comprehensive experiments and report the results in Table~\ref{tab:mathverse_test_result}. This analysis delves into the model's ability to address a broad spectrum of mathematical challenges, ranging from geometry to functions. 
\yz{write the results}



\begin{table*}[!t]
\small
\centering
\begin{adjustbox}{width=\linewidth}
    \begin{tabular}{l|c|cccccc|cccc|ccccc}
    \toprule
    \multirow{3}*{\makecell*[l]{\large Model}}    &\multirow{3}*{\makecell*[c]{All}}
    &\multicolumn{6}{c|}{\makecell*[c]{\shortstack{Plane Geometry}}} 
    &\multicolumn{4}{c|}{\makecell*[c]{\shortstack{Solid Geometry}}}
    &\multicolumn{5}{c}{\makecell*[c]{\shortstack{Functions}}}\\
    % \midrule
    \cmidrule{3-17}
    & &\makecell*[c]{All} &\makecell*[c]{Len} &\makecell*[c]{Area} &\makecell*[c]{Angle} &\makecell*[c]{Anal} &\makecell*[c]{Apply} &\makecell*[c]{All} &\makecell*[c]{Len} &\makecell*[c]{Area} &\makecell*[c]{Vol} &\makecell*[c]{All} &\makecell*[c]{Coord} &\makecell*[c]{Prop} &\makecell*[c]{Exp} &\makecell*[c]{Apply} \\
    \midrule
    \multicolumn{17}{c}{\textit{Closed-source MLLMs}}\\
    \cmidrule{1-17}
    Qwen-VL-Plus&21.3&17.3&19.1&16.4&16.1&23.6&13.2&24.8&18.1&18.7&33.4&31.3&52.5&25.1&10.8&50.3\\
    Gemini-Pro & 35.3 & 33.0 & 32.2 & 42.6  & 28.4 & 30.2 & 32.3 & 33.4 & 35.0 & 29.3 & 36.1  & 28.3 & 25.7  & 26.6& 10.8  & 51.3 \\
    Qwen-VL-Max & 37.2 & 38.4 & 41.7 & 46.4  & 32.6 & 40.6 & 38.7 & 33.7 & 25.4 & 28.3 & 42.6  & 38.4 & 43.7  & 35.5& 13.6  & 61.0 \\
    GPT-4V & {54.4} & {56.9} & {60.8} & {63.4}  & {52.6} & {48.5} & {60.9} & {50.2} & {54.8} & {39.9} & {56.8} & {52.8} & {72.3}  & {47.1} & {30.9}  & {70.1} \\
    \cmidrule{1-17}
    \multicolumn{17}{c}{\textit{Open-source MLLMs}}\\
    \cmidrule{1-17}
    LLaMA-Adapter V2&5.8 & 5.9&4.0&5.9&6.6&13.4&3.3&4.6&5.3&3.1&5.7&6.2&6.7&6.1&4.5&7.9\\
    ImageBind-LLM & 10.0& 9.7&12.1&9.9&9.2&10.2&4.8&4.6&4.9&3.5&5.3&14.9&12.3&13.8&4.6&25.9 \\
    mPLUG-Owl2 &10.3& 7.7&8.2&6.0&5.7&12.4&10.6&11.0&9.2&6.7&15.7&17.4&22.8&18.6&5.3&22.2\\
    
    MiniGPT-v2 &10.9&11.6&10.0&9.8&14.3&9.1&11.8&1.7&2.2&1.6&0.5&11.2&4.2&15.7&4.0&21.1\\
    LLaVA-1.5 & 12.7 & 11.8 & 13.1 & 15.1 & 9.7 & 9.4 & 13.2 & 10.6 & 12.1 & 8.7 & 11.6  & 14.8 & 18.8  & 12.7& 9.5  & 23.7\\
    SPHINX-Plus &14.0&14.4&14.2&10.5&14.1&16.5&16.8&7.0&7.2&6.1&7.6&17.9&11.1&19.1&6.3&27.7 \\
    G-LLaVA & 15.7 & 20.2 & 17.3&13.6&{26.5}&5.9&23.1&5.0&10.3&4.4&3.1&9.2&9.1&9.1&1.3&15.5\\
    LLaVA-NeXT & 17.2 & 15.9 & 14.8 & 13.1  & 16.3 & 17.7 & 17.8 & 19.6 & 33.3 & 11.7 & 12.6  & 23.1 & {24.5}  & 23.4 & 8.0  & 33.1\\
    ShareGPT4V &17.4&16.9&16.2&17.9&16.9&12.2&21.1&15.0&13.6&10.9&19.7&20.2&19.9&22.2&8.4&25.8\\
    SPHINX-MoE & 22.8 & 24.5 & 26.3 & 28.4  & 21.1 & {26.6} & {24.4} & 15.8 & 9.4 & 10.7 & {26.3}  & 19.5 & 23.5  & 19.3& 9.2  & 30.3\\
    InternLM-XC2 & {25.9} & {26.2} & {27.1} & {29.7}  & 20.6 & 18.5 & 22.2 & {20.1} & {34.5} & {14.1} & 25.2  & {23.7} & 24.4  & {24.9} & {10.6}  & {36.3}\\
    \cmidrule{1-17}
    \textbf{\model-9B}  \\
    \textbf{\model-19B} \\
    \textbf{\model-32B} \\
    \bottomrule
    \end{tabular}
\end{adjustbox}
\caption{\textbf{Mathematical Evaluation on Different Subjects and Subfields in MathVerse's \textit{testmini} Set.} We report the scores averaging five problem versions except for the `Text Only' version, and employ the CoT evaluation strategy by default. Len: Length; Anal: Analytic; Apply: Applied; Vol: Volume; Coord: Coordinate; Prop: Property; Exp: Expression; Apply: Applied. The highest accuracy for {closed-source} and {open-source} MLLMs is marked in red and blue respectively.}
\label{tab:mathverse_test_result}
\end{table*}




\vpara{Results on MathVision datasets.} To effectively assess \model's ability across diverse subjects and difficulty levels within the MathVision dataset, we conduct a series of detailed evaluation experiments and report results in Table~\ref{tab:mathvision_test_result}. \yz{write results}

\begin{table*}[htbp]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|c|cccccccccccccccc}
\toprule
\multicolumn{18}{c}{Human Performance}\\
\midrule
Model & Overall & Alg & AnaG & Ari & CombG & Comb & Cnt & DescG & GrphT & Log & Angle & Area & Len & SolG & Stat & Topo & TransG \\
\toprule
Random Chance & 7.17 & 1.5 & 11.9 & 7.1 & 9.7 & 4.8 & 6.0 & 22.1 & 1.1 & 7.6 & 0.6 & 9.4 & 6.7 & 8.2 & 8.6 & 13.0 & 7.1 \\
\midrule
Human (testmini) & 75.66 & 57.9 & 79.0 & 100.0 & 100.0 & 47.4 & 94.7 & 89.5 & 63.2 & 63.2 & 36.8 & 52.6 & 73.7 & 89.5 & 89.5 & 100.0 & 73.7 \\
\midrule
\multicolumn{18}{c}{LLMs (Text Only)}\\
\midrule
GPT4-CoT & 8.16 & 12.8 & 10.7 & 15.7 & 4.9 & 10.7 & 10.5 & 1.9 & 5.6 & 8.4 & 8.1 & 6.2 & 8.7 & 8.6 & 3.5 & 4.4 & 4.8	\\
\midrule
\multicolumn{18}{c}{LLMs (Text + Image Caption)}\\
\midrule
ChatGPT 3.5-CoT & 9.74 & 10.7 & 20.0 & 18.6 & 10.1 &7.7 & 17.9 & 16.4 & 10.0 & 13.5 & 6.4 & 5.8 & 6.5 & 9.4 & 12.1 & 4.4 & 10.7 \\	
GPT 4-CoT &13.10 & 16.5 & 20.2 & 34.3 & 10.4 & 17.9 & 19.4 & 7.7 & 11.1 & 10.1 & 9.8 & 9.6 & 9.1 & 13.5 & 13.8 & 8.7 & 12.5\\
\midrule
\multicolumn{18}{c}{Open-source LMMs (Text + Image)}\\
\midrule
LLaVA-v1.5-7B & 8.52 & 7.0 & 7.1 & 10.7 & 7.1 & 4.8 & 10.5 & 7.7 & 10.0 & 9.2 & 15.6 & 10.2 & 9.8 & 5.3 & 8.6 & 4.4 & 4.8 \\
SPHINX (V2) & 9.70 & 6.7 & 7.1 & 12.9 & 7.5 & 7.7 & 6.0 & 9.6 & 16.7 & 10.1 & 11.0 & 11.8 & 12.5 & 8.2 & 8.6 & 8.7 & 6.0 \\
ShareGPT4V-7B & 10.53 & 5.5 & 3.6 & 12.9 & 10.1 & 4.8 & 7.5 & 11.5 & 14.4 & 10.9 & 16.2 & 11.8 & 12.3 & 9.8 & 15.5 & 17.4 & 11.3 \\
LLaVA-v1.5-13B & 11.12 & 7.0 & 14.3 & 14.3 & 9.1 & 6.6 & 6.0 & 13.5 & 5.6 & 13.5 & 10.4 & 12.6 & 14.7 & 11.5 & 13.8 & 13.0 & 10.7 \\
ShareGPT4V-13B & 11.88 & 7.5 & 15.5 & 16.4 & 10.7 & 8.9 & 9.0 & 11.5 & 8.9 & 7.6 & 11.6 & 13.0 & 17.4 & 10.3 & 8.6 & 8.7 & 12.5 \\
SPHINX-MoE & 14.18 & 7.8 & 17.9 & 14.3 & 15.6 & 9.5 & 11.9 & 12.5 & 15.6 & 12.6 & 16.2 & 15.6 & 17.8 & 13.5 & 12.1 & 8.7 & 16.1 \\
InternLM-XComposer2-VL & 14.54 & 9.3 & 15.5 & 12.1 & 15.3 & 11.3 & 10.5 & 14.4 & {22.2} & {19.3} & {19.7} & 15.6 & 15.0 & 11.9 & 15.5 & {26.1} & 15.5 \\
\midrule
\multicolumn{18}{c}{Closed-source LMMs (Text + Image)}\\
\midrule
Qwen-VL-Plus & 10.72 & 11.3 & 17.9 & 14.3 & 12.7 & 4.8 & 10.5 & 15.4 & 8.9 & 14.3 & 11.6 & 6.4 & 10.0 & {14.3} & 6.9 & 8.7 & 11.31 \\
Qwen-VL-Max & 15.59 & 10.7 & {19.1} & 20.0 & 16.9 & {12.5} & {17.9} & 16.4 & 12.2 & {21.0} & 13.3 & 14.2 & 19.8 & 11.5 & {20.7} & 13.0 & 17.3 \\
Gemini Pro & {17.66} & {15.1} & 10.7 & {20.7} & {20.1} & 11.9 & 7.5 & {20.2} & {21.1} & 16.8 & 19.1 & {19.0} & {20.0} & {14.3} & 13.8 & 17.4 & {20.8} \\
GPT4V & {22.76} & {27.3} & {32.1} & {35.7} & {21.1} & {16.7} & {13.4} & {22.1} & 14.4 & 16.8 & {22.0} & {22.2} & {20.9} & {23.8} & {24.1} & {21.7} & {25.6} \\
\midrule
\textbf{\model-9B}  \\
\textbf{\model-19B} \\
\textbf{\model-32B} \\
\bottomrule
\end{tabular}%
}
\caption{Comparison of model performances across various mathematical subjects. Subjects: Alg: algebra, AnaG: analytic geometry, Ari: arithmetic, CombG: combinatorial geometry, Comb: combinatorics, Cnt: counting, DescG: descriptive geometry, GrphT: graph theory, Log: logic, Angle: metric geometry - angle, Area: metric geometry - area, Len: metric geometry-length, SolG: solid geometry, Stat: statistics, Topo: topology, TransG: transformation geometry. }
\label{tab:mathvision_test_result}
\end{table*}



\subsection{Generalizability of \model}

% Here, we compare our \model with conventional SOTA methods~\cite{} in geometry problem solving domain. Table~\ref{tab:conventional_results} demonstrates the comparisons between \model and several conventional models on the GeoQA and Geometry3K test dataset. Details description of several conventional SOTA methods are provided in Appendix~\ref{appendix: conventional_gps}. 

The proposed Math-LLaVA model has demon- strated exceptional performance in multimodal mathematical reasoning tasks. To assess its gener- alization capability, we conduct evaluation experi- ments using the MMMU benchmark, which encom- passes various disciplines and domains. The results are shown in Table 2. With only the selected data, Math-LLaVA has a performance drop on science subset. However, we can observe that the Math- LLaVA model fine-tuned on MathV360K can sig- nificantly outperforms the base model, LLaVA-1.5- 13B, as well as several other open-source MLLMs on all six sub-domains. This superior performance underscores its capability to generalize to down- stream multimodal understanding and reasoning tasks. Furthermore, the fine-tuning process using our synthetic data does not detract from the model’s reasoning abilities in other domains; rather, it en- hances its generalizability.

% \begin{table}[hbpt]
%     \centering
%     \renewcommand{\arraystretch}{1.15}
%     \setlength{\tabcolsep}{2mm}{
%     \begin{tabular}{c|cccc}  
%     \toprule
%       &  Model  & Input & GeoQA & Geometry3K   \\
%     % \midrule
%     % Random Chance & - & 25.0   \\
%     % Frequent Guess & - & 32.1   \\
%     \midrule
%     \multirow{3}{*}{\textit{Top-10 Accuracy}} &
%     NGS  &  \textit{Q}, \textit{I}  & 56.9 \\
%     & DPE-GPS &  \textit{Q}, \textit{I}  & 62.7 \\
%     & SCA-GPS &  \textit{Q}, \textit{I} & 64.1 \\
%     \midrule 
%     \multirow{7}{*}{\textit{Top-1 Accuracy}} & 
%      Geoformer  &  \textit{Q}, \textit{I} & 46.8 \\
%     & UniMath  &  \textit{Q}, \textit{I} & 50.0\\
%     & G-LLaVA-7B &  \textit{Q}, \textit{I} & 64.2\\
%     & G-LLaVA-13B &  \textit{Q}, \textit{I} & 67.0 \\
%     \cmidrule{2-5}
%     & \textbf{\model-9B}  &  \textit{Q}, \textit{I}\\
%     & \textbf{\model-19B} &  \textit{Q}, \textit{I}\\
%     & \textbf{\model-32B} &  \textit{Q}, \textit{I} \\
%     \bottomrule
%     \end{tabular}} 
%     \vspace{1cm}
%     \caption{Comparison between \model and conventional models on the GeoQA and Geometry3K test dataset.}
%     \label{tab:conventional_results}
% \end{table}



\begin{table}[hbpt]
    \centering
    \renewcommand{\arraystretch}{1.15}
    \resizebox{\textwidth}{!}{%    
    \begin{tabular}{c|c|cccccc}  
    \toprule
    Model  & MMMU & Art \& Design & Business & Sci. & Health \& Med. & Human. \& Social Sci. & Tech. \& Eng.   \\
    \midrule
    Random Chance  & 22.1 & 29.2 & 24.7 & 18.0 & 20.7 & 20.0 & 21.4 \\
    Frequent Guess & 26.8 & 23.3 & 29.3 & 27.3 & 30.0 & 25.8 & 24.8 \\
    miniGPT4-7B & 26.8 & 29.2 & 21.3 & 28.7 & 30.7 & 29.2 & 23.8 \\
    mPLUG-Owl-7B & 32.7  &	45.8 &	24.7&	22.7&	32.0&	45.8&	31.0 \\
    SPHINX-13B & 32.9&	48.3&	24.7&	26.7&	30.7&	50.0&	26.2 \\
    InstructBLIP-7B & 32.9& 	40.0& 	28.0& 	\textbf{32.7}& 	28.7& 	47.5& 	27.1 \\
    LLaVA-1.5-13B  & 36.4&	51.7&	22.7&	29.3&	38.7&	53.3&	31.4  \\
    \midrule
    \textbf{\model-9B} \\
    \textbf{\model-19B} \\
    \textbf{\model-32B} \\
    \bottomrule
    \end{tabular}} 
    \vspace{1cm}
    \caption{Comparison between \model and conventional models on the GeoQA and Geometry3K test dataset.}
    \label{tab:conventional_results}
\end{table}

\subsection{Further Analysis}




\vpara{Effect of Chinese Pre-training Dataset.} We validate the effectiveness of the adopted pre-training Chinese dataset. Table~\ref{tab:effect_data} \yz{write results}

\begin{table}[htbp]
    \centering
    \renewcommand{\arraystretch}{1.15}
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{c|ccc|cccccccccc}
        \toprule
      \multirow{2}{*}{Model}   & \multicolumn{3}{c|}{MathVista} &  \multicolumn{10}{c}{MathVision} \\
      & GPS & GEO & AVG & AnaG & CombG & DescG & GrphT & Angle & Area & Len & SolG & TransG & AVG \\
      \midrule
      GLM-4V-9B &  \\
      + SFT on English Data &  \\
      \midrule
      \model-9B   &   \\
         \bottomrule
    \end{tabular}}
    \vspace{0.2cm}
    \caption{Effect of the chinese pre-training dataset.}
    \label{tab:effect_data}
\end{table}



\vpara{Effect of VQA Datasets.} We validate the effectiveness of the adopted pre-training Chinese dataset. Table~\ref{tab:vqa_dataset} \yz{write results}

\begin{table}[htbp]
    \centering
    \renewcommand{\arraystretch}{1.15}
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{c|ccc|cccccccccc}
        \toprule
      \multirow{2}{*}{Model}   & \multicolumn{3}{c|}{MathVista} &  \multicolumn{10}{c}{MathVision} \\
      & GPS & GEO & AVG & AnaG & CombG & DescG & GrphT & Angle & Area & Len & SolG & TransG & AVG \\
      \midrule
      GLM-4V-9B &  \\
      + SFT on English Data &  \\
      \midrule
      \model-9B   &   \\
         \bottomrule
    \end{tabular}}
    \vspace{0.2cm}
    \caption{Effect of the VQA datasets.}
    \label{tab:vqa_dataset}
\end{table}


\subsection{Error Analysis}


We meticulously analyze the causes of errors in \model-32B and illustrate the distribution of these errors in Figure~\ref{fig:error_dist}. \yz{error analysis}

Detailed examples of these errors can be found in Appendix~\ref{appendix: error_cases}.


The most prevalent cause of errors, accounting for 42.2\%, was identified as Reasoning Error. This indicates a significant challenge in the model’s logical processing and inferential reasoning capabilities. Following closely, Vision Recognition Error was the second most common issue, responsible for 31.9\% of errors. This highlights difficulties in accurately interpreting visual data, suggesting that the vision encoder remains a bottleneck in multi-modal models. Knowledge Error, making up 15.1\% of the total errors, pointed to gaps in the model’s information database or its application. Furthermore, Calculation Error accounted for the smallest percentage of errors at 1.3\%, indicating that GPT-4V is relatively robust in numerical and computational tasks, which historically have been challenging for language models. Notably, all errors in the Calculation Error category related to symbolic computation, as shown in Figure~\ref{fig:error_one_case}, rather than numerical computation, suggesting a potential area for future improvement.

% \begin{figure}[hbpt]
%     \centering
%     \includegraphics[width=0.78\textwidth]{figs/error_dist.png}
%     \vspace{-2mm}
%     \caption{Error distribution of \model-32B on the \data.}
%     \label{fig:error_dist}
%     \vspace{-3mm}
% \end{figure}


% \begin{figure}[hbpt]
%     \centering
%     \includegraphics[width=0.78\textwidth]{figs/error_case.png}
%     \vspace{-2mm}
%     \caption{A typical calculation error.}
%     \label{fig:error_one_case}
%     \vspace{-3mm}
% \end{figure}



\begin{figure}[h]
\centering
\begin{minipage}{.5\textwidth}
  \centering
  \includegraphics[width=0.98\linewidth]{figs/error_dist.png}
  \captionof{figure}{Error distribution of \model-32B on the \data.}
  \label{fig:error_dist}
\end{minipage}%
\begin{minipage}{.5\textwidth}
  \centering
  \includegraphics[width=0.98\linewidth]{figs/error_case.png}
  \captionof{figure}{A typical calculation error.}
  \label{fig:error_one_case}
\end{minipage}
\end{figure}



